Dataset Distillation via Knowledge Distillation: Towards Efficient Self-Supervised Pre-Training of Deep Networks

Dataset distillation (DD) generates small synthetic datasets that can efficiently train deep networks with a limited amount of memory and compute. Despite the success of DD methods for supervised learning, DD for self-supervised pre-training of deep models has remained unaddressed. Pre-training on unlabeled data is crucial for efficiently generalizing to downstream tasks with limited labeled data. In this work, we propose the first effective DD method for SSL pre-training. First, we show, theoretically and empirically, that naive application of supervised DD methods to SSL fails, due to the high variance of the SSL gradient. Then, we address this issue by relying on insights from knowledge distillation (KD) literature. Specifically, we train a small student model to match the representations of a larger teacher model trained with SSL. Then, we generate a small synthetic dataset by matching the training trajectories of the student models. As the KD objective has considerably lower variance than SSL, our approach can generate synthetic datasets that can successfully pre-train high-quality encoders. Through extensive experiments, we show that our distilled sets lead to up to 13% higher accuracy than prior work, on a variety of downstream tasks, in the presence of limited labeled data. Code at https://github.com/BigML-CS-UCLA/MKDT.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}% Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The abstract and introduction claim that we propose an effective method for DD for SSL pre-training that can outperform baselines by up to 8\%. This is verified in the experiments section.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: In the experiments section, we discuss how these distilled sets, while improving upon baselines, cannot effectively train very large networks. We confjecture this is due to the small size of the distilled set, leading to the larger networks overfitting, rather than learning generalizable representations. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Proposition \ref{prop:var} is accompanied with detailed description of the data distribution, loss function and models considered to prove that the variance of 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provided detailed description of the setting in the main paper and exact hyper-parameters in the appendix. We also provide code to reproduce the results in the supplemental submission. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}
    \item[] Justification: The datasets we use are all public and we provide all code used in our paper in the supplemental submission.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: All experimental details are clearly explained in the experiments section and the appendices.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Standard deviations are reported for all results in the paper. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: These details are reported in the Appendix. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification: Yes, we confirm with the NeurIPS code of ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}
    \item[] Justification: We discuss the potential societal impact of this work in the Appendix. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    \item[] Justification: The models and data presented in this paper does not have a high risk of misuse. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have cited all datasets and methods we have used in this work. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}
    \item[] Justification: No new assets are released by this paper. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}
    \item[] Justification: No crowdsourcing experiments or research with human subjects is conducted for this paper. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: No crowdsourcing experiments or research with human subjects is conducted for this paper. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}


==> introduction.tex <==
\section{Introduction}


Dataset distillation (DD) aims to generate a very small set of synthetic images that can simulate training on a large image dataset, with extremely limited memory and compute \cite{dd_orig}. This facilitates training models on the edge, speeds up continual learning, 
% neural architecture search, hyper-parameter tuning, 
and provides strong privacy guarantees \cite{idc,mtt,sajedi2023datadam,dong2022privacy}. As a result, there has been a surge of interest in developing better DD methods for training neural networks in a supervised manner. %\cite{idc,mtt,sajedi2023datadam,chen2023data}. 
%%%%%%%%%%%%%%%%%
However, in many applications it is crucial to adapt the model quickly to \textit{new tasks} \cite{ben2006analysis}. In this case, supervised models often fail to generalize well. Instead, models are pre-trained on a large amount of \textit{unlabeled} data. Such models can be adapted quickly to several new tasks by simply training a linear classifier on a small number of labeled examples of each downstream task \cite{chen2023project,kirichenko2022last}. 
% This enables transferability to a variety of downstream tasks by training a linear model on the 
%%%%
% Self-supervised pre-training is much more expensive than supervised learning, but provides numerous benefits, including better transferability to new tasks \cite{?}, robustness against noisy labels \cite{?}, and superior out-of-distribution generalization performance \cite{?}. 
Nevertheless, DD for self-supervised pre-training has remained an open problem.

\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figs/dd_ssl.png}
    \vspace{-5mm}
    \caption{Dataset Distllation for SSL Pre-Training}
    \label{fig:ssl_dd}
    \vspace{-5mm}
\end{figure}

DD for SSL is, however, very challenging. One needs to ensure that pre-training on the synthetic dataset, distilled from unlabeled data, results in a encoder that yields high-quality representations for a variety of downstream tasks. Existing DD methods for SL generate synthetic data by matching gradients \cite{zhao_dc, zhao_dsa, dcc} or trajectory \cite{mtt, ftd, tesla} of training on real, distribution of real data \cite{dm,sajedi2023datadam, cafe}, or meta-model matching by generating synthetic data such that training on it achieves low loss on real data \cite{dd_orig,kip, rfad, frepo}. Among them, gradient and distribution matching methods heavily rely on labels and will suffer from representation collapse otherwise. Hence, they are not applicable to SSL DD.
% Several existing DD methods, including those that rely on gradient matching \cite{zhao_dc, zhao_dsa, dcc} and distribution matching \cite{dm,?} heavily rely on labels to generate the synthetic data. 
% Most DD methods for supervised learning, including %meta model matching \cite{?}, 
% gradient matching \cite{?}, and distribution matching \cite{?} generate a synthetic set of examples for every class in the original dataset. Having labels is essential for these methods, as otherwise the models trained on the synthetic data suffer from representation collapse and cannot distinguish examples in different classes. 
Very recently, \citet{lee2023selfsupervised} applied meta-model matching to generate synthetic examples for SSL pre-training, and evaluated its performance by {fine-tuning} the pre-trained model on full target datasets. However, pre-training on these distilled sets does not provide a significant advantage over pre-training on random examples, when evaluated by linear probe, as we confirm experimentally. This shows that the encoders cannot learn high-quality representations from the training data. \looseness=-1

% and the benefit is mainly resulted from fine-tuning, as we confirm experimentally. This is because kernel ridge regression using a fixed (or relatively unchanging) feature map cannot model the feature learning process of pre-training with SSL. Hence, synthetic examples generated by meta-model matching do not significantly change form their random initialization and cannot recover the rich features learnt on the real data. 

%This is because self-supervised learning (SSL) is generally much \textit{slower} than supervised learning. Hence, synthetic examples generated by meta model matching does not significantly change from their random initialization and cannot train the network far from its initialization.

In this work, we address distilling small synthetic datasets for SSL pre-training via trajectory matching. First, we show that na\"ive application of trajectory matching to SSL fails, due to the high variance of the gradient of the SSL loss. Then, we rely on insights from \textit{knowledge distillation} (KD) to considerably reduce the variance of SSL trajectories. KD trains a smaller student network %with superior performance over supervised learning by  training a student network 
to match the predictions of a larger teacher network trained with supervised learning \cite{hinton2015distilling}. In doing so, the student network can match the performance of the larger teacher model. First, we utilize this observation by training a student {encoder} to match the \textit{representations} of a larger teacher {encoder} trained with SSL. 
%that is trained in a self-supervised manner provides a superior performance over SSL. 
Then, we propose generating synthetic data for SSL by {M}atching {K}nowledge {D}istillation {T}rajectories (\method).
Crucially, as the KD objective for training the student model has considerably lower variance, it enables generating higher-quality synthetic data by matching the lower-variance trajectories of the \textit{student} model. 
% this approach has a crucial benefit for DD: it can train the student network much \textit{faster} than self-supervised techniques such as contrastive learning. 
%%%%%%%%%
As a result, the encoder can learn high-quality representations from the synthetic data.
%In our work, we generate synthetic subsets by matching the trajectories of the student model, without relying on labels. 

We conduct extensive experiments to validate the effectiveness of our proposal \method\ %: \textbf{M}atching \textbf{K}nowledge \textbf{D}istillation \textbf{T}rajectories for for distilling small synthetic datasets 
for SSL pre-training. In particular, we distill both low resolution (CIFAR10, CIFAR100) and high resolution datasets (TinyImageNet) down to 1\% and 5\% of original dataset size and show that, across various downstream tasks, \method\ distilled sets lead to 8\% higher accuracy. Moreover, we confirm that the datasets distilled with ConvNets can transfer to other larger architectures such as ResNets. Finally, we investigate the images distilled with our method and show that visually they appear to augment the primary object of the images, while distorting irrelevant information, conforming with our expectations of effective distilled datasets. 
% Thus, they enable effective dataset distillation for SSL pre-training. 


% we leverage trajectory matching to generate small synthetic subsets for pre-training neural networks with better transferability to target datasets, evaluated by linear probing. To generate such subsets,

% can be divided into the following categories: meta model matching generates synthetic data such that the model trained on the synthetic data generalizes well on the original dataset \cite{?}; gradient matching generates synthetic data to match the gradient of the model trained on the original dataset \cite{?}; trajectory matching generates synthetic data to match the weight trajectory of model trained on the original dataset \cite{?}; and distribution matching generates synthetic data to match the gradient of the model trained on the original dataset \cite{?}. 

==> notation.tex <==

\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}

==> old_related_work.tex <==
\section{Related Work}

\textbf{rewrite related work to be shorter and talk about how only meta-model matching and MTT can directly be used for SSL, but then discuss the challenges of both.}

\textbf{Ideally, talk about how meta-model matching is just not possible?}

Dataset distillation has been studied extensively for supervised learning, and the approaches can be broadly characterized into meta-model matching, gradient matching, distribution matching and trajectory matching \citep{sachdeva2023data}. Despite extensive research in these areas, there remains a gap in understanding how these methods can be adapted for contrastive learning.

\textbf{Meta-Model Matching.} Meta-model matching aims to maximize the performance of the model trained on the synthetic dataset $S$ when generalized
to the original dataset, with the objective function

\begin{equation}
\underset{S}{\text{arg min}} \; \mathcal{L}_D (\theta^{S}) 
\quad \text{s.t.} \quad \theta^{S} \triangleq \underset{\theta}{\text{arg min}} \; \mathcal{L}_{S} (\theta)
\end{equation}

\citep{dd_orig, sachdeva2023data}. The traditional DD approach is computationally and memory inefficient due to the bilevel optimization. Thus, several Kernel-based methods \citep {kip, rfad, frepo} have been proposed to solve the inner-loop in closed form, thus achieving better optimization. When applying to the contrastive learning setting, however, performing linear regression over a fixed feature map instead of feature learning cannot be used to explain and model the feature learning process of neural networks. \citep{pmlr-v139-wen21c}. 

\textbf{Gradient Matching. } Besides using Kernel-based methods, surrogate objectives have been proposed to resolve the inefficiency of the traditional DD. Gradient matching aims the gradient of the network trained on the target dataset and the gradient of the
network trained on the synthetic dataset. In particular, DC \citep{zhao_dc} match the gradients with respect
to the network weights giving real and synthetic data.
DSA \citep{zhao_dsa} built upon it to generate more informative synthetic datasets through siagmese augmentation for both
real and synthetic datasets. DCC \citep{dcc} proposes a roposed class-collective gradient matching, arguing that the class-wise
gradient matching strategy in DC and DSA overlooks the
contrastive signals between the classes, so are ineffective
for fine-grained image classification tasks.

All the gradient-matching distillation is done class-wise, making it easy to optimize the distillation objective. Thus, this method is not applicable to self-supervised learning where labels are not obtainable. In addition, the variance of gradients across mini-batches is too
large to be practical due to the contrastive loss depending on the examples in the batch. Thus, maintaining consistency between the original and distilled
data can be challenging due to this variability. One may argue that since covariance determines the gradient at any point, if we preserve the cross-covariance, we can do gradient matching efficiently \citep{tian2022understanding}. However, we are not sure whether this contrastive covariance is preserved as it largely depends on the batches that we sampled. [This is from a conversation with Sid before but I am not sure about this and we haven't discussed this further about it. I will look more into it]

\textbf{Trajectory Matching.} Trajectory matching aims to match the training trajectories of models trained on target dataset and synthetic dataset. MTT \citep{mtt} was the first trajectory matching proposed, and was improved upon by TESLA\citep{tesla} and FTD \citep{du2023minimizing} in terms of memory efficiency and robustness respectively. Due to the memory inefficiency of the original MTT, it is hard to be applied to self-supervised case, as self-supervised learning in general needs larger number of epochs of training compared with supervised learning. This results in large amount of synthetic steps in the inner loop of MTT and results in large computation graph accumulating up in memory. The longer training trajectory also makes already-existing gradient vanishing problem in MTT \citep{idc} more severe for contrastive learning. In addition, the batch-wise gradient calculation makes the trajectory matching objective hard to be optimized. In [Section x], we empirically and theoretically show that trajectory matching cannot be applied effectively to contrastive learning.

\textbf{Distribution Matching.} Distribution matching directly match the distribution for synthetic dataset and target dataset. In DM \citep{dm}, the synthetic data are optimized to match the original data distribution in a family of embedding spaces by using the maximum mean discrepancy (MMD). CAFE \citep{cafe} maintains both real-feature distribution and the discrepancy of the synthetic dataset. IDM \citep{zhao2023improved} improves upon DM by partitioning and expansion augmentation, efficient model sampling, and class-aware distribution regularization. The distribution matching approach also relies on labels, which is unobtainable for self-supervised learning. However, if we use certain methods (e.g., Kmeans) which divides the dataset into clusters, distribution matching applies as the loss function only considers the distribution of the embeddings of the synthetic and real data, and is unrelated to the type of learning algorithm.

\textbf{Add-on to Existing Data Distillation Methods.} factorization methods expand datasets using techniques like multiformations \citep{idc}. As \cite{sachdeva2023data} discussed, factorization differs fundamentally from other dataset distillation methods where each synthesized data point is maintained as a set of free parameters. In addition, DREAM \citep{liu2023dream} and DREAM+ \citep{liu2023dream+} selects representative original images to be matched with. 
PDD \citep{chen2023data} distills data progressively by synthesizing multiple small sets, with each each conditioned on the previous sets. All those methods can be integrated into the dataset distillation techniques above. 


\textbf{Data-Efficient Learning for Contrastive Learning} Another method for data-efficient learning is coreset selection \citep{mirzasoleiman2020coresets, paul2021deep}. While it is also widely studied for supervised learning, \cite{pmlr-v202-joshi23b} proposes a way to selects subsets of real-data to enable data-efficient contrastive learning by selecting subsets that maximize augmentation similarity to the full dataset. Our work instead focuses on creating a small synthetic dataset such that training on this smaller dataset is equivalent to performance to training on the larger
full dataset. KRR-ST \citep{anonymous2023selfsupervised} was first proposed as a self-supervised data distillation method for transfer learning that tries to find a distilled set such that model trained on it with a SSL objective achieves low SSL loss on the full dataset, and used kernel-based method to avoid the costly bilevel optimization. This method also avoid the biased gradient of data distillation for SSL by avoiding data augmentation and using full batch in the training process.









% \textbf{SELF-SUPERVISED DATASET DISTILLATION FOR TRANSFER LEARNING}

% \textit{Setting
% }


% \begin{itemize}
% \item Self-supervised data distillation for transfer learning: distill $\rightarrow$
%  pre-train a model on the distilled data $\rightarrow$
%  fine-tune on the target task. What we do is distill $\rightarrow$
%  linear evaluation for a randomly initialized model on the distilled dataset.

%  \item Use Barlow Twins for SSL

% \item They target on the issue of biased estimator with gradient matching using SSL and ensure an unbiased estimator for the true gradient.

% - Source of bias: data augmentation; randomness of batch
% - (?)but what if only data augmentation and randomness are the sources of bias, can you just not do augmentation in gradient matching approach and use supervised CL to avoid augmentation. This only explains self supervised learning but not contrastive learning as a whole. We can also argue about the variance (for samples from real data); Also did not show why contrastive loss is harder to optimize
% \end{itemize}

% \textit{Method
% }
% \begin{itemize}

% \item basic idea is to match the representation of the model trained on synthetic data with that of the model trained on real data, and during the training procedure they didn't do data augmentation and used full batch, thus eliminating randomness


% \item First pre-train on full dataset with SSL, get $g\phi$
%  (this can be expensive)
% \item inner loop - minimize MSE between a model representation of synthetic samples $X_s$
%  and target representations $Y_s$ (both are optimized in the outer loop - target representation is also learnable?) - get $\hat{g}_{\theta}$
% \item outer loop - MSE between the original data representation of the model from inner loop $\hat{g}_{\theta^*}(X_t)$
%  and that of the model pre-trained on the original dataset $g\phi(X_t)$.
% \item split the model into a feature extractor and a linear head, freeze the feature extractor (could be a problem) and optimize only the linear head with KRR during the inner optimization 
% \begin{itemize}
%     \item So they still need this expensive bilevel optimization and to optimize it they replace it with KRR but that comes to the problem for using kernel-based approach unable to model feature learning process.
% \end{itemize}
% \begin{itemize}
%     \item they assume a linear head but many of the projection heads are nonlinear.
%     \item Need diverse models to prevent overfitting
% \end{itemize}

% \end{itemize}

% \textit{baseline experiments
% }

% \begin{itemize}
% \item Transfer learning, Architecture Generalization, and data-free knowledge distillation
% \item Used the original experiment setup to do pretraining + fine-tune. Didn't replace the supervised learning with contrastive learning for network update.

%  \end{itemize}





% \textbf{Dataset Distillation by Meta-Model Matching} \citep{dd_orig, kip, kip_conv}

% \textit{\textbf{Why they might not work}}
% \begin{itemize}
% \item extreme long trajectories needed to train contrastive learning to convergence (inner loop too long). And even for the kernel-based approach which aims to not do the unrolling of the inner-loop at each outer-loop update, it still requires storing all computational graphs and a heavy matrix inversion operation so difficult to scale \citep{tesla}. 
% \item kernel-based approaches: not valid because NTK approach cannot be used to explain or model the feature learning process of neural networks as it does linear regression over a fixed feature map instead of feature learning.  \citep{pmlr-v139-wen21c}. 
% \item NTK operates under the assumption of a linearized approximation in a fixed feature space. If NTK is used to distill data for training a contrastive learning model, it might fail to capture the non-linearities and complexity of the embedding space developed during contrastive learning
% \end{itemize}

% \textit{\textbf{Methods in the Category}}
% \begin{itemize}
% \item DD: network parameters as a function of synthetic data and learn them through the network parameters to minimize the training loss over the original data
% \item KIP/RFAD/FrePO \textbf{(SOTA)}: kernel-based approach
% \end{itemize}

% \textbf{Dataset Distillation by Gradient Matching}

% \textit{\textbf{Why they might not work}}
% \begin{itemize}
%     \item gradient distillation is done class-wise to make the distillation objective more tractable i.e. without this it is hard to optimize the distillation objective.
    
%     % \cite{jiang2022delving} proposes to match the multi-level gradients to involve both intra-class and inter-class gradient information using different classes but this is similar to DCC
%     \item As mentioned in \cite{cafe}, the majority of gradients might arise mainly from a select set of challenging examples or noise, thus gradient matching may overlook those representative but easy samples, while overfit to those hard samples or noises. Also, variations can exist in the hard examples that produce large gradients across different network architectures, so reliance solely on gradients might not generalize well to unseen architectures (Since the hard examples may vary across different architectures). The problems will be more severe in the case of contrastive learning.
%     \item even if had labels, contrastive learning on a batch of examples from same class would actually be harmful, your batch only has false negatives
%     \begin{itemize}
%         \item Could also use Supervised CL and In-Batch Negative Sampling but 
%         \begin{itemize}
%             \item In terms of robustness: The objective of gradient matching is to maintain a similar gradient dynamic as the original data, but we might focus too much on approximating the gradients and potentially neglecting to preserve the intra-class and inter-class variances in the data.  
%             \item Optimal sampling is crucial: We want to have enough negative samples in the batch for CL itself to be meaningful, thus let the distilled images to also learn this and be balanced and diverse enough. Also we want distilled data not to be biased towards specific classes or clusters in the feature space 
%         \end{itemize}
%     \end{itemize}
%     \item if we were to gradient matching with random batches, the variance of gradients across mini-batches is too large to be practical due to the contrastive loss depending on what examples are put together in a batch. Maintaining consistency between the original and distilled data can be challenging due to this variability
%     \item Augmentation.
%      \item Preserve covariance? \cite{tian2022understanding} proposes that gradient descent for contrastive loss is equivalent to gradient ascent of $\mathcal{E}_{\alpha}(\theta) := \frac{1}{2} \text{tr}\left(C_{\alpha}[z(\theta), z(\theta)]\right)$ where the contrastive covariance $C_{\alpha}[a, b] := \sum_{i=1}^{N} \sum_{j \neq i} \alpha_{ij} (a[i] - a[j])(b[i] - b[j])^T - \sum_{i=1}^{N} \left( \sum_{j \neq i} \alpha_{ij} \right) (a[i] - a[i'])(b[i] - b[i'])^T$. Here $\alpha_{ij}(\theta) := \phi'(s_i) \psi'(d_i^2 - d_{ij}^2)$, characterizing the pairwise importance. However, we are not sure whether this contrastive covariance is preserved since $\alpha$ depends on the batches.



% \end{itemize}

% \textit{\textbf{Methods in the Category}}
% \begin{itemize}
% \item DM / DSA - DM match the gradients with respect to the network weights giving real and synthetic data. DSA built upon DM to generate more informative synthetic datasets through siagmese augmentation for both real and synthetic; both focus on class-wise gradient + periodic model initialization


% \item DCC / DSAC \textbf{(SOTA)} - Argues that the class-wise gradient matching strategy in DM / DSA overlooks the contrastive signals between the classes, so ineffective for fine-grained image classification tasks; want to enable the optimization of a synthetic dataset to capture the contrastive signals. Proposed class-collective gradient matching but still are matching class wise, they just sum it up. 
% \end{itemize}

% \textbf{Dataset Distillation by Trajectory Matching}

% Have empirically shown that the loss function is harder to optimize for CL. Also we need to train for longer trajectories to see meaningful results, so the gradient vanishing problem is more significant for CL than for standard supervised learning. In addition, we have more aggressive augmentation for CL. 

% \textbf{Dataset Distillation by Distribution Matching} \textbf{NOT SOTA}

% Aims to avoid the expensive bi-level optimization. The assumption is that two datasets which are similar according to a particular distribution divergence metric, also lead to similarly trained models \citep{sachdeva2023data}. Here the type of learning doesn't matter as the loss function only considers the distribution of the embeddings of the synthetic and real data. 

% \textit{\textbf{Why they might work}}
% \begin{itemize}
% \item Match the mean features of the real and synthetic image batche and ensures that the data distribution (in terms of class balance, feature dynamics, etc.) of the distilled dataset matches as closely as possible to that of the original dataset. if the original dataset is representative and robust in terms of CL.
% \item Distribution matching might help to retain examples that are particularly important or difficult, ensuring that the distilled dataset still provides complex and informative learning signals.
% \end{itemize}

% \textit{\textbf{Why they might not work}}
% \begin{itemize}
% \item matches distribution class-wise and requires labels. 
% \item \cite{cafe} proposes a way to encode the discriminant capabilities into the synthetic samples. However, while it will preserve inter-class variability, might not maintain intra-class variability.
% \item Also if the matching is not class-wise, distribution matching does not necessarily ensure balanced batch compositions. Matching the global data distribution doesn’t necessarily guarantee that the local batch-wise distributions are similarly matched

% \end{itemize}

% \textit{\textbf{Methods in the Category}}
% \begin{itemize}
% \item DM: the synthetic data are optimized to match the original data distribution in a family of embedding spaces by using the maximum mean discrepancy (MMD)
% \item CAFE: two objectives: 1. data distribution alignment: match features that involve all internediary layers. 2. discrimination: reals samples as testing sample and classify based on the synthetic clusters. It also uses a bi-level optimization scheme to alleviate underfitting and overfitting, and thus both the synthetic data and network are updated. So the type of learning algorithm matters here. 
% \item IDM \citep{zhao2023improved} \textbf{(SOTA)}: argues that for traditional DM, the features of the distilled dataset scatter around, causing severe class misalignment problems. The number of features for distilled dataset is too small, and you're trying to represent a large, possibly varied feature space with a significantly reduced one. Proposed partitioning and expansion augmentation. They also regularize the feature distribution of distilled datasets to alleviate class misalignment 




% \end{itemize}

% \textbf{Factorization} As discussed in \cite{sachdeva2023data}, factorization methods are not directly comparable to other dataset distillation methods that maintain each synthethized data point as set of free-parameters as factorization methods expand out factorized datasets using e.g. multiformations \citep{idc} etc. to get larger effective datasets. 



% \textbf{Data-Efficient Learning for Contrastive Learning}

% More closely related to our work is \citep{pmlr-v202-joshi23b} that selects subsets of real-data to enable data-efficient contrastive learning. Our work instead focuses on creating a small synthetic dataset such that training on this smaller dataset is equivalent to performance to training on the larger full dataset. 

==> scratch.tex <==
\section{Introduction}
Goal: how to dataset distilll for SSL 
Immediate thinking: MTT since it doesn't require any class information. (DM / DC etc. all require class informaiton)

\subsection{Potential pitches for this paper}
\begin{itemize}
    \item What to distill for SSL is SAS
    \begin{itemize}
        \item pros:
        \begin{itemize}
            \item works well with thesis / prior work 
            \item simple to run 
        \end{itemize}
        \item cons:
        \begin{itemize}
            \item setting to beat KRRST = small proxy model 
        \end{itemize}
    \end{itemize}
    \item What to distill for SSL is high loss (same for SL) even for small IPC, if you use MSE loss and soft-labels (logits of SL model / representations from model trained with SSL )
    \begin{itemize}
        \item pros:
        \begin{itemize}
            \item seems like this will work and is useful for both SL and SSL 
        \end{itemize}
        \item cons:
        \begin{itemize}
            \item not very relevant to SSL necessarily so motivation is a little iffy if we focus on SSL distillation
\item not as related to thesis
        \end{itemize}
    \end{itemize}
    \item Adapting SL distillation to SSL 
    \begin{itemize}
        \item pros:
        \begin{itemize}
            \item very simple to do
            \item results are already good
        \end{itemize}
        \item cons:
        \begin{itemize}
            \item lack of novelty
        \end{itemize}
    \end{itemize}
\end{itemize}

\subsection{Motivation for SSL distillation.}
\begin{itemize}
    \item SSL allows us to use large amounts of unlabeled data and learn representations that can generalize to various downstream tasks.  
    \item SSL representations are evaluated using linear probe i.e. training a linear classifier on the representations learnt by the model trained with SSL
    \item These linear classifiers can be trained with very little labeled data. 
    \item However, a major downside of SSL is the large amount of pre-training (unlabeled) data needed $\rightarrow$ high cost of training
    \item Dataset distillation's goal is to create a small synthetic dataset to mimic a larger real dataset i.e. training on the smaller dataset leads to similar performance as training on the larger real dataset
    \item this is the first dataset distillation method for SSL 
    \item prior work has studied dataset distillation for sup learning and studied dataset distillation for transfer learning.  goal is different.
    \item our baselines will be: 
    \begin{enumerate}
        \item directly doing end-to-end SL on the small amount of labeled data we have
        \item random subset of unlabeled data + LP with small labeled data
        \item KRRST
        \item our method (MTT + initializing with high loss examples + distilling high loss examples)
    \end{enumerate}
\end{itemize}

Additional information about the setting includes having access to the CIFAR100 dataset with all unlabeled data, as well as 10 labeled points per class or a total of 1000 labeled points from different downstream datasets such as CIFAR100 and CIFAR10. The objective is to perform semi-supervised learning (SSL) on the CIFAR100 dataset and subsequently utilize the randomly selected labeled points for label propagation (LP) purposes.

For the SSL part, we are going to dataset distillation, to make the pre-training more efficient. 

Source dataset: CIFAR100
Downstream datasets: CIFAR100, CIFAR10
Number of Labeled Points per Downstream datasets: 10 images per class
Pre-training on Synthetic: 50 epochs


\begin{table*}[h]
    \centering
    \begin{tiny}
    \begin{tabular}{|c|c|l|c|l|c|l|l|l|} \hline  
         &  Direct SL&   Full Data SSL&Random  &High Loss 60\%&  High Loss Subset&KRRST (Random)&KRRST (High Loss) &Best Us So Far \footnote{(MTT + Trajectories trained on high loss examples i.e. what to distill + Initialized syn images as high loss examples)}\\ \hline  
         CIFAR100&  14.6&   30.34&21.92 &&  21.07&22.43& 22.63&23.7\\ \hline  
 CIFAR100 (full LP)& & & 42 &52& & 46& &48.15\\ \hline 
         CIFAR10&  26&   &35.47 &&  37.53&37.82& 38.72&39.8\\ \hline  
 CIFAR10 \footnote{(100 labeled images available per class)}& &  &53.05 && 52.94& 53.68& 54.93&55.23\\ \hline 
 CIFAR10 (full LP)& & &  && & 70.22& &71.79\\ \hline
    \end{tabular}
    \end{tiny}
    \caption{Caption (Sid)}
    \label{tab:my_label}
\end{table*}


\begin{table}
    \centering
    \begin{tabular}{ccc}
         Method&  CIFAR100 (1000 LP)& CIFAR100 (full LP)\\
         train on random init&  20.8& \\
 train on high loss init& 20.98&44.01\\
         low loss 40pct, random init&  22.13& 45.93\\
         low loss 60pct, random init&  21.8& 46.15\\
         high loss, random init&  22.5& 46.27\\
 high loss, high loss init& 24.06&47.77\\
 all, random init& 24.5&48.6\\
 all, high loss init& 24.95&48.19\\
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}


\begin{table*}
    \centering
    \begin{tabular}{|c|c|l|} \hline 
         Subset& C100 100\% labels LP &1000 Labels LP\\ \hline 
         Full Data&  52.64&30.34\\
 Original Model& 65.42&52.94\\\hline \hline 
         High Loss 60\% (Large IPC)& 52.2 &28.82\\ \hline 
         High Loss 2\%&  39.71&16.71\\ \hline 
         Low Loss 60\%& 51.31 &\\ \hline 
 Low Loss 2\%& 36.8&14.37\\ \hline
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table*}

\clearpage


\begin{table}[h!]
  \centering
  \begin{tabular}{lc}
    \toprule
    Method & Linear Eval Acc. \\
    \midrule
    KRRST (SAS init) & 50.590 \\
    KRRST (random init) & 49.420 \\
    SAS subset & 55.610 \\
    \bottomrule
  \end{tabular}
  \caption{CIFAR10}
  \label{tab:my_label}
\end{table}



\begin{table*}[h]
\centering
\begin{small}
\begin{tabular}{llcccccc}
\toprule
\multirow{2}{*}{Size (\%)} & \multirow{2}{*}{Method} & \multicolumn{1}{c}{Source} & \multicolumn{5}{c}{Target} \\
\cmidrule(lr){3-3} \cmidrule(lr){4-8}
& & C10 & C100 & Aircraft & CUB2011 & Dogs & Flowers \\
\midrule
& No Pre-Training & 60.35$\scriptstyle{\pm 0.24}$ & 33.43$\scriptstyle{\pm 0.40}$ & 23.12$\scriptstyle{\pm 0.33}$ & 7.46$\scriptstyle{\pm 0.18}$ & 9.33$\scriptstyle{\pm 0.18}$ & 22.52$\scriptstyle{\pm 0.75}$ \\
\midrule
\multirow{3}{*}{0.5\%} & Random Subset & 61.80$\scriptstyle{\pm 0.16}$ & 36.71$\scriptstyle{\pm 0.15}$ & 23.56$\scriptstyle{\pm 0.18}$ & 8.78$\scriptstyle{\pm 0.07}$ & 9.75$\scriptstyle{\pm 0.07}$ & 27.33$\scriptstyle{\pm 0.51}$ \\
& KRR-ST & x & x & x & x & x & x \\
& \method\ & 65.93$\scriptstyle{\pm 0.14}$ & 38.94$\scriptstyle{\pm 0.29}$ & 25.99$\scriptstyle{\pm 0.31}$ & 9.02$\scriptstyle{\pm 0.37}$ & 10.51$\scriptstyle{\pm 0.12}$ & 27.66$\scriptstyle{\pm 0.44}$ \\
\midrule
\multirow{3}{*}{1\%} & Random Subset & 62.31$\scriptstyle{\pm 0.19}$ & 37.46$\scriptstyle{\pm 0.17}$ & 23.77$\scriptstyle{\pm 0.07}$ & 9.4$\scriptstyle{\pm 0.07}$ & 9.71$\scriptstyle{\pm 0.36}$ & 29.53$\scriptstyle{\pm 0.15}$ \\
& KRR-ST & 65.58$\scriptstyle{\pm 0.33}$ & 39.6$\scriptstyle{\pm 0.51}$ & 24.65$\scriptstyle{\pm 0.640}$ & 9.81$\scriptstyle{\pm 0.28}$ & 10.37$\scriptstyle{\pm 0.07}$ & 29.24$\scriptstyle{\pm 0.33}$ \\
& \method\ & \textbf{66.92}$\scriptstyle{\pm 0.32}$ & \textbf{40.75}$\scriptstyle{\pm 0.17}$ & \textbf{27.08}$\scriptstyle{\pm 0.74}$ & \textbf{10.09}$\scriptstyle{\pm 0.12}$ & \textbf{10.79}$\scriptstyle{\pm 0.17}$ & \textbf{30.47}$\scriptstyle{\pm 0.10}$ \\
\midrule
100\% & Full Data & R $\scriptstyle{\pm x}$ & R $\scriptstyle{\pm x}$ & R $\scriptstyle{\pm x}$ & R $\scriptstyle{\pm x}$ & R $\scriptstyle{\pm x}$ & R $\scriptstyle{\pm x}$ \\
\bottomrule
\end{tabular}
\caption{\textbf{SIMCLR} Linear Probe, CIFAR10 Pre-training (Full)}
\label{tab:comparison}
\end{small}
\end{table*}

\begin{table*}[h]
\centering
\begin{small}
\begin{tabular}{llcccccc}
\toprule
\multirow{2}{*}{Size (\%)} & \multirow{2}{*}{Method} & \multicolumn{1}{c}{Source} & \multicolumn{5}{c}{Target} \\
\cmidrule(lr){3-3} \cmidrule(lr){4-8}
& & C100 & C10 & Aircraft & CUB2011 & Dogs & Flowers \\
\midrule
& No Pre-Training & 33.43$\scriptstyle{\pm 0.40}$ & 60.35$\scriptstyle{\pm 0.24}$ & 23.12$\scriptstyle{\pm 0.33}$ & 7.46$\scriptstyle{\pm 0.18}$ & 9.33$\scriptstyle{\pm 0.18}$ & 22.52$\scriptstyle{\pm 0.75}$ \\
\midrule
\multirow{3}{*}{1\%} & Random Subset & x & x & x & x & x & x \\
& KRR-ST & x & x & x & x & x & x \\
& \method\ & x & x & x & x & x & x \\
\midrule
100\% & Full Data & R $\scriptstyle{\pm x}$ & R $\scriptstyle{\pm x}$ & R $\scriptstyle{\pm x}$ & R $\scriptstyle{\pm x}$ & R $\scriptstyle{\pm x}$ & R $\scriptstyle{\pm x}$ \\
\bottomrule
\end{tabular}
\caption{Linear Probe, ImageNet Pre-training}
\label{tab:comparison}
\end{small}
\end{table*}


\begin{table*}[h]
\centering
\begin{small}
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{1}{c}{Source} & \multicolumn{5}{c}{Target} \\
\cmidrule(lr){2-2} \cmidrule(lr){3-7}
Method & C100 & C10 & Aircraft & CUB2011 & Dogs & Flowers \\
\midrule
No Pre-Training & 33.59 & 60.08 & 22.65 & 7.28 & 9.58 & 22.44 \\
\midrule
Random Subset (1\%) & x & x & x & x & x & x \\
KRR-ST (1\%) & x & x & x & x & x & x \\
\method\ (1\%) & x & x & x & x & x & x \\
\midrule
Random Subset (5\%) & x & x & x & x & x & x \\
KRR-ST (5\%) & x & x & x & x & x & x \\
\method\ (5\%) & x & x & x & x & x & x \\
\midrule
Random Subset (10\%) & 43.28 & 67.22 & 28.29 & 10.46 & 10.57 & 33.16 \\
KRR-ST (10\%) & 46.07 & 69.88 & 27.90 & 10.87 & 12.39 & 35.37 \\
\method\ (10\%) & \textbf{48.59} & \textbf{71.07} & \textbf{29.49} & \textbf{12.17} & \textbf{12.61} & \textbf{38.69} \\
\bottomrule
\end{tabular}
\caption{Linear Probe, C100 Pre-training (Full)}
\label{tab:comparison}
\end{small}
\end{table*}


\begin{table*}[h]
\centering
\begin{small}
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{1}{c}{Source} & \multicolumn{5}{c}{Target} \\
\cmidrule(lr){2-2} \cmidrule(lr){3-7}
Method & C100 & C10 & Aircraft & CUB2011 & Dogs & Flowers \\
\midrule
No Pre-Training & 11.64 & 40.32 & 8.88 & 3.19 & 3.83 & 22.02 \\
\midrule
Random Subset (1\%) & x & x & x & x & x & x \\
KRR-ST (1\%) & x & x & x & x & x & x \\
\method\ (1\%) & x & x & x & x & x & x \\
\midrule
Random Subset (5\%) & x & x & x & x & x & x \\
KRR-ST (5\%) & x & x & x & x & x & x \\
\method\ (5\%) & x & x & x & x & x & x \\
\midrule
Random Subset (10\%) & 20.2 & 52.17 & 11.37 & 4.63 & 4.56 & 33.05 \\
KRR-ST (10\%) & 22.93 & 54.84 & 10.74 & 4.82 & 4.81 & 35.08 \\
\method\ (10\%) & \textbf{24.22} & \textbf{57.16} & \textbf{12.39} & \textbf{5.07} & \textbf{4.76} & \textbf{38.46} \\
\bottomrule
\end{tabular}
\caption{Linear Probe, C100 Pre-training (Few Shot)}
\label{tab:comparison}
\end{small}
\end{table*}













\begin{table*}[h]
\begin{small}
\begin{tabularx}{\textwidth}{@{}lXXX@{}} 
\toprule
Dataset & {No Pre-Training} & {us}  &  {regular KRR-ST} \\
\midrule
C100            & 48.94 & 50.58  & 50.61 \\
C100 (1000)     & 12.48 & 24.17  & 21.88 \\
C100 (100)      & 3.15  & 7.47     & 6.83  \\
C10             & 79.07 & 80.23 & 80.55 \\
C10 (1000)      & 45.84 & 58.76  & 57.14 \\
C10 (100)       & 24.0  & 39.16  & 36.26 \\
Aircraft        & 33.15 & 36.60   & 35.49 \\
Aircraft (1000) & 9.21  & 12.42  & 11.01 \\
Aircraft (100)  & 2.97  & 3.18     & 3.12  \\
CUB2011         & 11.36 & 15.52 & 13.69 \\
CUB2011(1000)   & 3.33  & 5.40     & 4.97  \\
CUB2011(100)    & 1.62  & 2.12     & 2.00  \\
Dogs            & 12.10 & 14.31  & 13.78 \\
Dogs (1000)     & 3.69  & 4.71   & 4.63  \\
Dogs (100)      & 1.95  & 2.19   & 2.34  \\
Flowers         & 23.86 & 40.14  & 35.42 \\
Flowers (1000)  & 23.56 & 39.97 & 35.53 \\
Flowers (100)   & 8.70  & 14.10 & 12.59 \\
\bottomrule
\end{tabularx}
\centering
\caption{Finetune, C100 pre-training}
\label{tab:finetune}
\end{small}
\end{table*}

\begin{table*}[h]
\centering
\begin{small}
\begin{tabularx}{\textwidth}{@{}lXXXX@{}} 
\toprule
Dataset & No pre-train & random 50 ipc & us & KRR-ST \\
\midrule 
C10             & 60.08      & 62.72         & 67.1            & 65.14               \\ 
C10 (1000)      & 40.32      & 45.41         & 50.46           & 49.48              \\  
C10 (100)       & 23.97      & 30.69         & 33.89           & 34.85              \\ 
C100            & 33.59      & 37.55         & 40.99           & 39.68              \\ 
C100 (1000)     & 11.64      & 15.04         & 17.06           & 16.01              \\ 
C100 (100)      & 3.45       & 4.64          & 4.79            & 4.67               \\
Aircraft        & 22.65      & 23.52         & 27.39           & 24.78              \\ 
Aircraft (1000) & 8.88       & 9.42          & 11.04           & 10.08              \\ 
Aircraft (100)  & 3.36       & 3.45          & 3.33            & 3.03               \\ 
CUB2011         & 7.28       & 9.13          & 9.96            & 9.79               \\ 
CUB2011(1000)   & 3.19       & 4.02          & 4.28            & 4.30               \\ 
CUB2011(100)    & 2.00       & 2.04          & 2.14            & 2.26               \\ 
Dogs            & 9.58       & 9.64          & 11.19           & 10.90              \\ 
Dogs (1000)     & 3.83       & 3.90          & 4.31            & 4.09               \\ 
Dogs (100)      & 2.02       & 2.35          & 2.44            & 2.38               \\
Flowers         & 22.44      & 28.61         & 29.97           & 30.13              \\ 
Flowers (1000)  & 22.02      & 28.52         & 29.78           & 29.89              \\ 
Flowers (100)   & 9.06       & 10.83         & 11.77           & 11.52              \\
\bottomrule
\end{tabularx}
\caption{LP, C10 pre-training}
\label{tab:finetune}
\end{small}
\end{table*}

\begin{table*}[h]
\begin{small}
\begin{tabularx}{\textwidth}{@{}lXXXX@{}} 
\toprule
Dataset & {No Pre-Traiining} & {random 50 ipc} & {us} & {distilled (KRR-ST)} \\
\midrule
C100            & 49.01 & 47.69 & 48.31 & R \\
C100 (1000)     & 12.53 & 15.27 & 16.81 & R \\
C100 (100)      & 3.15  & 3.97  & 4.65  & R \\
C10             & 79.42 & 78.51 & 79.19 & R \\
C10 (1000)      & 45.82 & 48.23 & 52.60 & R \\
C10 (100)       & 24.0  & 26.77 & 35.44 & R \\
Aircraft        & 33.24 & 32.34 & 34.65 & R \\
Aircraft (1000) & 9.27  & 9.72  & 11.10 & R \\
Aircraft (100)  & 2.94  & 3.27  & 3.51  & R \\
CUB2011         & 11.27 & 11.37 & 12.53 & R \\
CUB2011(1000)   & 3.33  & 4.14  & 4.38  & R \\
CUB2011(100)    & 1.62  & 2.30  & 2.21  & R \\
Dogs            & 12.04 & 11.66 & 12.89 & R \\
Dogs (1000)     & 3.68  & 4.02  & 4.34  & R \\
Dogs (100)      & 1.95  & 1.97  & 2.25  & R \\
Flowers         & 23.87 & 28.87 & 30.59 & R \\
Flowers (1000)  & 23.58 & 28.49 & 30.22 & R \\
Flowers (100)   & 8.68  & 10.54 & 11.76 & R \\
\bottomrule
\end{tabularx}
\centering
\caption{FT: C10 Pre-training}
\label{tab:yourlabel}
\end{small}
\end{table*}



\begin{table}[h!]
  \centering
  \begin{tabular}{lc}
    \toprule
    Method & Linear Eval Acc. \\
    \midrule
    Rand Subset & 47.75 \\
    SAS subset (Kmeans R10) & 47.9 \\
    SAS subset (Original) & 50.1 \\
    SAS subset (Original) Distilled & running \\
    \bottomrule
  \end{tabular}
  \caption{CIFAR100 R18 (50 IPC)}
  \label{tab:my_label}
\end{table}

DM: refers to matching representations by minimizing MSE between mean of synthetic and real. 

Initialization for all the methods is SAS 10 ipc using kmeans. And the real data is SAS 50ipc using kmeans. 

\begin{table}[h!]
  \centering
  \begin{tabular}{lc}
    \toprule
    Method & Linear Eval Acc. \\
    \midrule
    Rand Subset & J \\
    SAS subset (Kmeans R50) & J \\
    Random Networks DM  & S \\
    Trained Network DM & S \\
    Hidden Layer Random Networks DM & S \\
    Hidden Layer Trained Network DM  & S \\
    SAS subset (Original) & J \\
    \bottomrule
  \end{tabular}
  \caption{CIFAR100 R18 (10 IPC)}
  \label{tab:my_label}
\end{table}




\sj{CIFAR100
\begin{itemize}
    \item Run 1\% and 5\% which is 500 and 2500 images 
\end{itemize}
}






\begin{table*}[h]
\centering
\begin{small}
\begin{tabular}{llcccccc}
\toprule
\multirow{2}{*}{Size (\%)} & \multirow{2}{*}{Method} & \multicolumn{1}{c}{Source} & \multicolumn{5}{c}{Target} \\
\cmidrule(lr){3-3} \cmidrule(lr){4-8}
& & C10 & C100 & Aircraft & CUB2011 & Dogs & Flowers \\
\midrule
& No Pre-Training & 60.35$\scriptstyle{\pm 0.24}$ & 33.43$\scriptstyle{\pm 0.40}$ & 23.12$\scriptstyle{\pm 0.33}$ & 7.46$\scriptstyle{\pm 0.18}$ & 9.33$\scriptstyle{\pm 0.18}$ & 22.52$\scriptstyle{\pm 0.75}$ \\
\midrule
\multirow{3}{*}{1\%} & Random Subset & 63.32$\scriptstyle{\pm 0.19}$ & 37.40$\scriptstyle{\pm 0.04}$ & 23.23$\scriptstyle{\pm 0.42}$ & 8.81$\scriptstyle{\pm 0.12}$ & 9.86$\scriptstyle{\pm 0.20}$ & 26.83$\scriptstyle{\pm 0.43}$ \\
& KRRST & 64.55$\scriptstyle{\pm 0.32}$ & 37.13$\scriptstyle{\pm 0.17}$ & 24.21$\scriptstyle{\pm 0.17}$ & 8.53$\scriptstyle{\pm 0.06}$ & 10.30$\scriptstyle{\pm 0.36}$ & 26.23$\scriptstyle{\pm 0.65}$ \\
& \method\ & 65.52$\scriptstyle{\pm 0.07}$ & 39.52$\scriptstyle{\pm 0.33}$ & 25.60$\scriptstyle{\pm 0.54}$ & 9.60$\scriptstyle{\pm 0.30}$ & 10.69$\scriptstyle{\pm  0.10}$ & 29.19$\scriptstyle{\pm 0.19}$ \\
\midrule
\multirow{3}{*}{5\%} & Random Subset & 68.0$\scriptstyle{\pm 0.29}$ & 41.41$\scriptstyle{\pm 0.16}$ & 26.60$\scriptstyle{\pm 0.25}$ & 10.12$\scriptstyle{\pm 0.28}$ & 10.95$\scriptstyle{\pm 0.18}$ & 31.63$\scriptstyle{\pm 0.14}$ \\
& KRRST & x & x & x & x & x & x \\
& \method\ & 70.31$\scriptstyle{\pm 0.19}$ & 43.83$\scriptstyle{\pm 0.34}$ & 30.24$\scriptstyle{\pm 0.97}$ & 10.97$\scriptstyle{\pm 0.42}$ & 11.55$\scriptstyle{\pm 0.12}$ & 34.25$\scriptstyle{\pm 0.58}$ \\
\midrule
100\% & Full Data & R $\scriptstyle{\pm x}$ & R $\scriptstyle{\pm x}$ & R $\scriptstyle{\pm x}$ & R $\scriptstyle{\pm x}$ & R $\scriptstyle{\pm x}$ & R $\scriptstyle{\pm x}$ \\
\bottomrule
\end{tabular}
\caption{Linear Probe, CIFAR10 Pre-training (Full)}
\label{tab:comparison}
\end{small}
\end{table*}





\begin{table*}[h]
\centering
\begin{small}
\begin{tabular}{llcccccc}
\toprule
\multirow{2}{*}{Size (\%)} & \multirow{2}{*}{Method} & \multicolumn{1}{c}{Source} & \multicolumn{5}{c}{Target} \\
\cmidrule(lr){3-3} \cmidrule(lr){4-8}
& & C100 & C10 & Aircraft & CUB2011 & Dogs & Flowers \\
\midrule
& No Pre-Training & 33.43$\scriptstyle{\pm 0.40}$ & 60.35$\scriptstyle{\pm 0.24}$ & 23.12$\scriptstyle{\pm 0.33}$ & 7.46$\scriptstyle{\pm 0.18}$ & 9.33$\scriptstyle{\pm 0.18}$ & 22.52$\scriptstyle{\pm 0.75}$ \\
\midrule
\multirow{3}{*}{1\%} & Random Subset & 37.44$\scriptstyle{\pm 0.19}$ & 62.42$\scriptstyle{\pm 0.21}$ & 23.57$\scriptstyle{\pm 0.63}$ & 8.84$\scriptstyle{\pm 0.25}$ & 10.03$\scriptstyle{\pm 0.15}$ & 27.41$\scriptstyle{\pm 0.42}$ \\
& KRRST & 37.36$\scriptstyle{\pm 0.32}$ & 63.42$\scriptstyle{\pm 0.21}$ & 24.22$\scriptstyle{\pm 0.40}$ & 8.39$\scriptstyle{\pm 0.35}$ & 10.49$\scriptstyle{\pm 0.17}$ & 26.60$\scriptstyle{\pm 0.11}$ \\
& \method\ & 39.28$\scriptstyle{\pm 0.55}$ & 64.41$\scriptstyle{\pm 0.24}$ & 25.33$\scriptstyle{\pm 0.59}$ & 9.50$\scriptstyle{\pm 0.15}$ & 10.42$\scriptstyle{\pm 0.22}$ & 28.92$\scriptstyle{\pm 0.26}$ \\
\midrule
\multirow{3}{*}{5\%} & Random Subset & 42.10$\scriptstyle{\pm 0.04}$ & 66.52$\scriptstyle{\pm 0.22}$ & 26.90$\scriptstyle{\pm 0.67}$ & 9.95$\scriptstyle{\pm 0.32}$ & 10.87$\scriptstyle{\pm 0.24}$ & 32.68$\scriptstyle{\pm 0.71}$ \\
& Low Loss Subset & 41.7 & x & x & x & x & x \\
& KRRST & x & x & x & x & x & x \\
& \method\ & 44.73$\scriptstyle{\pm 0.19}$ & 68.87$\scriptstyle{\pm 0.56}$ & 29.29$\scriptstyle{\pm 0.29}$ & 11.72$\scriptstyle{\pm 0.25}$ & 11.48$\scriptstyle{\pm 0.08}$ & 37.12$\scriptstyle{\pm 0.45}$ \\
% \midrule
% \multirow{3}{*}{10\%} & Random Subset & 43.62$\scriptstyle{\pm 0.32}$ & 67.57$\scriptstyle{\pm 0.28}$ & 28.03$\scriptstyle{\pm 0.37}$ & 10.53$\scriptstyle{\pm 0.07}$ & 10.94$\scriptstyle{\pm 0.26}$ & 33.17$\scriptstyle{\pm 0.40}$ \\
% & KRRST & 46.15$\scriptstyle{\pm 0.28}$ & 70.25$\scriptstyle{\pm 0.11}$ & 27.93$\scriptstyle{\pm 0.47}$ & 10.30$\scriptstyle{\pm 0.15}$ & 12.10$\scriptstyle{\pm 0.18}$ & 34.99$\scriptstyle{\pm 0.34}$ \\
% & \method\ & \textbf{48.18}$\scriptstyle{\pm0.32}$ & \textbf{71.19}$\scriptstyle{\pm0.38}$ & \textbf{30.58}$\scriptstyle{\pm0.47}$ & \textbf{11.72}$\scriptstyle{\pm0.26}$  & \textbf{12.30}$\scriptstyle{\pm0.08}$ & \textbf{38.76}$\scriptstyle{\pm0.23}$ \\
\midrule
100\% & Full Data & R $\scriptstyle{\pm x}$ & R $\scriptstyle{\pm x}$ & R $\scriptstyle{\pm x}$ & R $\scriptstyle{\pm x}$ & R $\scriptstyle{\pm x}$ & R $\scriptstyle{\pm x}$ \\
\bottomrule
\end{tabular}
\caption{Linear Probe, CIFAR100 Pre-training (Full)}
\label{tab:comparison}
\end{small}
\end{table*}





\begin{table*}[h]
\centering
\begin{small}
\begin{tabular}{llccccccc}
\toprule
\multirow{2}{*}{Size (\%)} & \multirow{2}{*}{Method} & \multicolumn{1}{c}{Source} & \multicolumn{5}{c}{Target} \\
\cmidrule(lr){3-3} \cmidrule(lr){4-9}
& & Tiny ImageNet & C100 & C10 & Aircraft & CUB2011 & Dogs & Flowers \\
\midrule
& No Pre-Training & 14.26$\scriptstyle{\pm 0.16}$ & 33.43$\scriptstyle{\pm 0.40}$ & 60.35$\scriptstyle{\pm 0.24}$ & 23.12$\scriptstyle{\pm 0.33}$ & 7.46$\scriptstyle{\pm 0.18}$ & 9.33$\scriptstyle{\pm 0.18}$ & 22.52$\scriptstyle{\pm 0.75}$\\
\midrule
\multirow{3}{*}{1\%} & Random Subset & 18.56$\scriptstyle{\pm 0.12}$ & 34.92$\scriptstyle{\pm 0.31}$ & 61.71$\scriptstyle{\pm 0.46}$ & 23.47$\scriptstyle{\pm 0.20}$ & 7.49$\scriptstyle{\pm 0.29}$ & 9.71$\scriptstyle{\pm 0.15}$ & 23.16$\scriptstyle{\pm 0.29}$\\
& KRRST & 16.17$\scriptstyle{\pm 0.07}$ & 33.92$\scriptstyle{\pm 0.31}$ & 61.47$\scriptstyle{\pm 0.46}$ & 22.49$\scriptstyle{\pm 0.53}$ & 7.34$\scriptstyle{\pm 0.27}$ & 9.46$\scriptstyle{\pm 0.23}$ & 23.41$\scriptstyle{\pm 0.80}$\\
& \method\ & 20.14$\scriptstyle{\pm 0.01}$ & 36.90$\scriptstyle{\pm 0.18}$ & 63.43$\scriptstyle{\pm 0.25}$ & 24.36$\scriptstyle{\pm 0.24}$ & 8.41$\scriptstyle{\pm 0.46}$ & 10.31$\scriptstyle{\pm 0.17}$ & 25.59$\scriptstyle{\pm 0.26}$\\
% \midrule
% \multirow{3}{*}{5\%} & Random Subset & 25.45$\scriptstyle{\pm 0.19}$ & 38.15$\scriptstyle{\pm 0.09}$ & 66.44$\scriptstyle{\pm 0.34}$ & 25.59$\scriptstyle{\pm 0.28}$ & 8.78$\scriptstyle{\pm 0.20}$ & 10.83$\scriptstyle{\pm 0.28}$ & 25.61$\scriptstyle{\pm 0.25}$\\
% & KRRST & x & x & x & x & x & x \\
% & \method\ & x & x & x & x & x & x & x\\
\midrule
100\% & Full Data & R $\scriptstyle{\pm x}$ & R $\scriptstyle{\pm x}$ & R $\scriptstyle{\pm x}$ & R $\scriptstyle{\pm x}$ & R $\scriptstyle{\pm x}$ & R $\scriptstyle{\pm x}$ \\
\bottomrule
\end{tabular}
\caption{Linear Probe, Tiny ImageNet Pre-training}
\label{tab:comparison}
\end{small}
\end{table*}
\begin{table*}[t]
\centering
\begin{small}
\begin{tabular}{llccccccc}
\toprule
\multirow{2}{*} & \multirow{2}{*}{Method} & \multicolumn{1}{c}{Source} & \multicolumn{5}{c}{Target} \\
\cmidrule(lr){3-3} \cmidrule(lr){4-9}
& & C100 & Tiny ImageNet & C10 & Aircraft & CUB2011 & Dogs & Flowers \\
\midrule
& No Pre-Training  & 8.94$\scriptstyle{\pm 0.26}$ & 5.24$\scriptstyle{\pm 0.14}$ &  34.56$\scriptstyle{\pm 0.61}$ & 4.40$\scriptstyle{\pm 0.25}$ & 1.98$\scriptstyle{\pm 0.14}$ & 3.31$\scriptstyle{\pm 0.17}$ & 11.34$\scriptstyle{\pm 0.27}$ \\
\midrule
& Random Subset & 12.05$\scriptstyle{\pm 0.57}$ & 7.56$\scriptstyle{\pm 0.36}$ &  39.22$\scriptstyle{\pm 0.79}$ & 5.91$\scriptstyle{\pm 0.21}$ & 2.68$\scriptstyle{\pm 0.05}$ & 4.17$\scriptstyle{\pm 0.23}$ & 11.36$\scriptstyle{\pm 0.72}$ \\
& High Loss Subset & 16.39$\scriptstyle{\pm 0.79}$ & 10.43$\scriptstyle{\pm 0.40}$ &  44.26$\scriptstyle{\pm 0.53}$ & 7.77$\scriptstyle{\pm 0.35}$ & 4.28$\scriptstyle{\pm 0.57}$ & 5.44$\scriptstyle{\pm 0.32}$ & 14.65$\scriptstyle{\pm 1.11}$ \\
& KRR-ST & 11.52$\scriptstyle{\pm 0.15}$ & 7.34 $\scriptstyle{\pm 0.14}$ & 38.85$\scriptstyle{\pm 0.42}$ &5.79$\scriptstyle{\pm 0.17}$ & 2.70$\scriptstyle{\pm 0.07}$ & 4.00$\scriptstyle{\pm 0.01}$ & 10.50$\scriptstyle{\pm 0.29}$ \\
& \method\ & 12.29$\scriptstyle{\pm 0.01}$ & 7.81$\scriptstyle{\pm 0.09}$ & 39.46$\scriptstyle{\pm 0.46}$ & 6.13$\scriptstyle{\pm 0.24}$ & 2.66$\scriptstyle{\pm 0.06}$ & 4.11$\scriptstyle{\pm 0.05}$ & 12.25$\scriptstyle{\pm 0.38}$ \\
& \method\ (high loss) & 15.82$\scriptstyle{\pm 0.49}$ & 10.21$\scriptstyle{\pm 0.24}$ & 44.14$\scriptstyle{\pm 0.37}$ & 7.59$\scriptstyle{\pm 0.08}$ & 4.22$\scriptstyle{\pm 0.18}$ & 5.10$\scriptstyle{\pm 0.27}$ & 14.67$\scriptstyle{\pm 0.78}$ \\
\bottomrule
\end{tabular}
\caption{Linear Probe, CIFAR100 (5\%) AlexNet}
\label{tab:comparison}
\end{small}
\end{table*}


\begin{table*}[t]
\centering
\begin{small}
\begin{tabular}{llccccccc}
\toprule
\multirow{2}{*} & \multirow{2}{*}{Method} & \multicolumn{1}{c}{Source} & \multicolumn{5}{c}{Target} \\
\cmidrule(lr){3-3} \cmidrule(lr){4-9}
& & C100 & Tiny ImageNet & C10 & Aircraft & CUB2011 & Dogs & Flowers \\
\midrule
& No Pre-Training  & 8.6$\scriptstyle{\pm 0.21}$ & 7.15$\scriptstyle{\pm 0.26}$ &  27.43$\scriptstyle{\pm 0.20}$ & 4.25$\scriptstyle{\pm 0.17}$ & 1.34$\scriptstyle{\pm 0.14}$ & 2.02$\scriptstyle{\pm 0.10}$ & 3.58$\scriptstyle{\pm 0.20}$ \\
\midrule
& Random Subset & 6.49$\scriptstyle{\pm 0.19}$ & 5.96$\scriptstyle{\pm 0.28}$ &  29.57$\scriptstyle{\pm 0.76}$ & 3.41$\scriptstyle{\pm 0.17}$ & 1.82$\scriptstyle{\pm 0.06}$ & 2.74$\scriptstyle{\pm 0.20}$ & 4.46$\scriptstyle{\pm 0.18}$ \\
& High Loss Subset & 9.01$\scriptstyle{\pm 1.26}$ & 6.90$\scriptstyle{\pm 1.07}$ &  31.49$\scriptstyle{\pm 2.30}$ & 3.82$\scriptstyle{\pm 0.48}$ & 2.07$\scriptstyle{\pm 0.25}$ & 3.18$\scriptstyle{\pm 0.32}$ & 5.29$\scriptstyle{\pm 0.74}$ \\
& KRR-ST & 8.6$\scriptstyle{\pm 0.21}$ & 7.15$\scriptstyle{\pm 0.26}$ & 27.43$\scriptstyle{\pm 0.20}$ & 4.25$\scriptstyle{\pm 0.17}$ & 1.34$\scriptstyle{\pm 0.14}$ & 2.02$\scriptstyle{\pm 0.10}$ & 3.58$\scriptstyle{\pm 0.20}$ \\
& \method\ & x & x & x & x & x & x & x \\
& \method\ (high loss) x & x & x & x & x & x & x \\
\bottomrule
\end{tabular}
\caption{Linear Probe, CIFAR100 (5\%) VGG 11}
\label{tab:comparison}
\end{small}
\end{table*}















% In this section, we present how we effectively distill large real datasets into small synthetic datasets for SSL pre-training. In particular, we first present why trajectory-matching based distillation is more promising than other approaches such as gradient matching, distribution matching and meta-model matching. We then show why directly applying MTT to SSL is challenging. Finally, we present our proposal, \method, \textbf{M}atching \textbf{K}nowledge \textbf{D}istillation \textbf{T}rajectories, which relies on KD for SSL to adapt trajectory matching for SSL pre-training. 

%consider a trajectory matching based approach as trajectory matching is 1) agnostic to learning algorithm unlike gradient matching, distribution matching etc. and 2) can capture the feature learning of the encoder better than kernel-based meta-model matching. Since the goal of SSL is to learn encoders that can provide useful representations across a variety of downstream tasks, it is crucial for the distilled sets to capture the training dynamics of the encoder; however, meta-model matching using kernel-based approaches considers a fixed or relatively unchanging encoder and thus cannot do so effectively. 

%We then cover the challenges 

% In this section, we first show that the naive application of trajectory matching fails for SSL due to the high variance of the SSL objective's gradient. Then, we theoretically and empirically verify that the gradient for the knowledge distillation objective of a model trained with SSL has lower variance than training directly with SSL. Finally, we present the details of our method, \method\ (\textbf{M}atching \textbf{K}nowledge \textbf{D}istillation \textbf{T}rajectories), which operationalizes the above insight by: 1) training a large teacher encoder with SSL, 2) collecting trajectories of encoders trained with the KD objective using the teacher encoder and the full real data (\jn{I don't quite understand this part. it would be better if we mention clearly that the trajectory is trained by matching the encoder representation and the target representation}, and 3) optimizing the synthetic data to match the expert trajectories of KD on the full real data.
% In our investigation into methods for extending supervised learning distillation to self-supervised learning (SSL), we focus on two primary approaches: meta-model matching and trajectory matching, given that other methods hinge on class information.  \sj{why can DD not work}. Despite the challenges posed by the intractability of meta-model matching, recent endeavors to address this issue using kernel-based methods prove insufficient.  The inadequacy arises from the fact that kernel methods inherently assume a fixed feature map, neglecting the crucial aspect of optimizing synthetic sets dynamically for SSL's fundamental objective — learning encoders to extract generalizable features. 

% We confirm this through synthetic experiments i.e. training used a fixed (or slowly changing) feature map does not help the synthetic data train feature extractors that are as useful as those trained on the real data. Our experiment distills synthetic data using Kernelized Ridge Regression and varies the number of updates of the feature extractor (from 0 to large) for both SL and SSL. \sj{We find that training the feature extractor for more steps can lead to much larger improvements in the synthetic datasets distilled for SSL than SL, demonstrating that it is essential for a dataset distillation method for SSL to capture the properties of data useful for training feature extractors.} Potentially it is sufficient to show how much the weights of feature extractor change when we train on our synthetic set v/s when they train on theirs. 

% Consequently, we explore how to extend Matching Training Trajectories (MTT) \citep{mtt} to SSL.

% The primary objective of MTT is to optimize the synthetic dataset to capture long-range training dynamics of the real data. This is done by matching multiple training steps on distilled data with a significantly larger number of steps on the real dataset. In particular, MTT obtains "expert trajectories," representing the trajectories followed by models trained on the full real dataset. The key idea of MTT is to distill a dataset capable of inducing a trajectory similar to the expert trajectory (or trajectories) by optimizing the synthetic dataset to have similar weights as the model trained on the full data when starting from the same point (weights).

% \begin{itemize}
%     \item MTT can't work with SSL loss due to high variance of the gradient of SSL due to the loss depending on whole batch. 
%     \item as a result of this, convergence is much slower and many more steps are needed on both real and synthetic data to get meaningful trajectories (movement away from initialization) and trajectories are noisier
%     \item moreover, matching longer trajectories is extremely challenging due to the accumulated error in traj matching (look at how FTD describes this issue, if we can show methods like FTD too cannot fix this)
%     \item we empirically confirm this by 1) showing that from SSL trajectories trained from same initialization have higher variance than SL trajectories from same initialization 2) distillation for the high variance trajectories of SSL is less sucesssful (show plot of distillation loss over time)
%     \item As an alternative we propose using a simple knowledge distillation approach to train the expert trajectories i.e. train them to minimize MSE to representations of a much larger model.
%     \item theoretically, we show that this loss has much smaller variance than the SSL loss.
%     \item Moreover, this has the added benefit of training models that can outperform SSL training for the expert trajectories
% \end{itemize}

% \subsection{\sj{Appeal of Trajectory Matching for SSL}}

% In contrast to gradient matching, which aligns gradients \textit{class-wise} between synthetic and real data, and distribution matching, which similarly aligns data representations \textit{class-wise}, trajectory matching operates independently of labels.

% Meta-model matching is the only other dataset distillation method that does not rely on labels. However, its direct application in SL has been shown to be costly. This issue is even more pronounced in SSL, where the training costs for models are significantly higher \citep{}. Furthermore, while kernel-based meta-model matching is a more efficient alternative, it is ineffective for SSL. Since SSL aims to learn encoders that provide useful representations for various downstream tasks, it is vital for distilled sets to capture the training dynamics of the encoder. Kernel-based meta-model matching, which assumes a fixed or relatively static encoder, fails to do this effectively. In contrast, trajectory matching is capable of capturing these essential training dynamics.

% Therefore, trajectory matching stands out as the most promising approach for SSL dataset distillation.



% \textbf{SSL Objectives have High Variance Gradient.} SSL is known to have slower convergence than SL, which can be attributed to the high variance of gradients.
% %, requiring often requiring far more epochs than training with SL \citep{zbontar2021barlow, chen2020simple, grill2020bootstrap}.
% % For example, training a ResNet50 with Barlow Twins on ImageNet to convergence requires 1000 epochsas compared to training with SL that requires only 100 epoch \citep{zbontar2021barlow}. Other SSL methods \citep{chen2020simple, grill2020bootstrap} take similarly long to converge. 
% This high variance is caused by SSL losses being: 1) dependent on all examples in a batch, and 2) reliant on strong random augmentations. As shown in Eq. \eqref{eq:bt_loss}: the loss of a batch depends on the cross-correlation of representations of all examples within a batch. As a result, the contribution of each example to the loss can vary significantly depending on the other examples in the batch. This leads to high variance in gradients since batches are determined randomly. In SL, however, this is not the case. 
% % The loss of each example is determined solely by that example. Thus, regardless of other examples in the batch, a given example's contribution to the gradient will remain constant.
% Moreover, the use of stronger augmentations in SSL than in SL causes larger variance in the input to the model for SSL, and consequently, larger variance in the gradient. 
% In Fig. \ref{fig:high_var_traj}, we empirically confirm this for a 3-layer ConvNet. We train 5 SL and SSL models from the same initialization and record the average variance over all model parameters, while keeping all other hyperparameters (like learning rate, optimizer, etc.) identical for a fair comparison. The larger variance in parameters after 1 epoch of SGD when training with SSL compared to SL confirms that the variance of gradients for SSL is significantly larger.
 
% \textbf{High Variance Gradients Prevent Effective Trajectory Matching.} 

%We confirm this empirically in Fig. \ref{fig:high_var_traj_2}, where we show the variaince of the models trained with SSL and SL, using with different random seeds, on the full real data with identical initial weights and hyper-parameters. The large distillation loss illustrates that even with training on the full real data, trajectories of SSL vary far more than those with SL, showing how much noisier SSL trajectories are . This accumulated error in trajectory matching gets even larger with longer

% Moreover, the trajectories themselves are much noisier than SL due to the high variance of the gradient. As a result, the error accumulated while matching SSL trajectories as compared to matching SL trajectories of even equal length is much higher. Together, the need to match longer trajectories and the higher error in matching trajectories, makes directly applying trajectory matching to SSL ineffective. 

% In Fig. \ref{fig:explain:exp1}, we plot the variance in trajectories of increasing length when training with SL and SSL (\sj{SimCLR, BT}). Specifically, we train \textbf{X} \textbf{arch} for SL and SSL from the same initialization for \textbf{Y} epochs on \textbf{DATASET} and then compare the mean variance of each parameter across the \textbf{X} models after epochs 1 through \textbf{Y}. As we see in Fig. \ref{fig:explain:exp1} even for trajectories starting from the same initialization, the high variance in SSL gradient leads to much larger variance in the resulting trajectories and as trajectories get longer this variance increases faster for SSL than it does for SL. Through this experiment, we confirm that the trajectories of SSL are indeed noisier than those of SL and this worsens with longer trajectories. 

% In Fig. \ref{fig:explain:exp2}, we plot the distillation loss over iterations for SL and SSL. In particular, for both SL and SSL (\sj{SimCLR, BT}) we initialize our synthetic images as \textbf{Z} randomly selected real images and distill to match a single expert trajectory of length \textbf{Y}. Fig. \ref{fig:explain:exp2} shows that the distillation loss decreases much more rapidly for the SL trajectory matching objective, showing that even considering a single expert trajectory, matching the trajectory with the noisier SSL trajectory on the synthetic data is a much more challenging optimization than it is for SL. This simple experiment illustrates that matching the noisier synthetic data training trajectories of SSL with the noisier real data training trajectories of SSL would be even more challenging and unlikely lead to meaningful distilled images. 


% Contributions:
% Challenges with MTT for SSL (which has now been described in previous section)
% \begin{itemize}
%     \item SSL gradient has high variance (this is new, KRRST claims the meta-model matching bilevel optimization with SSL has biased gradient, this is very different from what we say)
%     \item High variance grad prevents effective traj matching
% \end{itemize}
% Solutions
% \begin{itemize}
%     \item Switch to KD for SSL 
% \end{itemize}

% In Fig. \ref{fig:high_var_traj}, \textit{KD Trajectories} refers to the variance of trajectories for 3-layer ConvNet, trained with the KD objective using a BarlowTwins ResNet-18 at the teacher encoder. 
 

% Training the expert trajectories using the knowledge distillation objective has the added benefit of resulting in encoders that are more effective than those trained using SSL directly. Thus, we adapt trajectory matching for dataset distillation for SSL by using the knowledge distillation objective of matching representations of a larger model. 

% As an alternative to training with SSL, we consider training with the KD objective (Eq. \eqref{eq:kd}) and a teacher encoder pre-trained with SSL. Importantly, this has 2 notable differences to training with the SSL loss: 1) the loss no longer depends on every example in a batch 2) there is no need to rely on (strong) augmentations for learning. Thus, we conjecture the variance of the gradient of this KD objective is significantly lower than that of SSL. We first prove this theoretically in Theorem \ref{thm:var_mse}, where for a simplified data distribution and linear models, we demonstrate that the variance of gradient of the KD objective is lower than that of the Barlow-Twins (SSL). 

% \begin{theorem} \label{thm:var_mse}
% Linear model, simple data distribution that resembles sparse coding model but is low dimensional.
% Var(MSE Loss) $<$ Var(Barlow Twins) \sj{fix}
% \end{theorem}
% Proof in Appendix \ref{app:proof}. 

% We also validate empirically that, as a consequence, the trajectories of training with KD are lower variance in Fig. \ref{fig:high_var_traj}. The empirical setup is the same as Sec. \ref{sec:mtt_ssl_fail} with KD training using a ResNet-18 trained with BarlowTwins.
